Analytical Prediction of Equilibrium Existence in Current-Limited Grid-Forming Inverters

As converter-interfaced units become dominant in power systems, understanding nonlinear stability phenomena involving discrete switching events becomes essential for secure operation. The limited overcurrent capability of grid-forming (GFM) inverters makes current limiting essential during large disturbances. Activation of a circular current limiter (CCL) can cause the operating equilibrium to disappear under certain circumstances. This paper develops an analytical framework to predict the grid-voltage boundaries for CCL activation and determine whether the operating equilibrium persists or disappears after activation. For CCL-based GFM inverters with frozen anti-windup, closed-form expressions for the activation boundaries are derived while accounting for the filter capacitor. A criterion is established to determine whether a saturated (i.e., current-limited) stable equilibrium point (satSEP) persists following limiter activation. A continuation method is also developed to trace equilibria across normal-control and current-limited operation. Power-angle analysis and dynamic-model continuation in single-inverter and modified 9-bus systems validate these predictions. Time-domain simulations further confirm the results. The results show that CCL activation can either cause immediate loss of the stable equilibrium or allow stable current-limited operation to continue until the equilibrium is lost as operating conditions change further.

==> tmpcite-1.tex <==
\cite{paquette_virtual_2015,lu_virtual-impedance-based_2018}


==> tmpcite-2.tex <==
\cite{liu_optimal_2021,sadeghkhani_current_2017}


==> tmpcite-3.tex <==
\cite{erckrath_voltage_2022}


==> tmpcite-4.tex <==
\cite{fan_fault_2023}


==> tmpcite-5.tex <==
\cite{arjomandi-nezhad_modeling_2025,li_transient_2023,lu_segmental_2024,me_transient_2023}


==> tmpcite-6.tex <==
\cite{arjomandi-nezhad_modeling_2025,li_transient_2023,lu_segmental_2024}


==> tmpcite-7.tex <==
\cite{ji_limit-induced_2025,zeng_dynamic_2026,ji_hidden_2026}

